Scratching Visual Transformer's Back with Uniform Attention

The favorable performance of Vision Transformers (ViTs) is often attributed to the multi-head self-attention (MSA). The MSA enables global interactions at each layer of a ViT model, which is a contrasting feature against Convolutional Neural Networks (CNNs) that gradually increase the range of interaction across multiple layers. We study the role of the density of the attention. Our preliminary analyses suggest that the spatial interactions of attention maps are close to dense interactions rather than sparse ones. This is a curious phenomenon, as dense attention maps are harder for the model to learn due to steeper softmax gradients around them. We interpret this as a strong preference for ViT models to include dense interaction. We thus manually insert the uniform attention to each layer of ViT models to supply the much needed dense interactions. We call this method Context Broadcasting, CB. We observe that the inclusion of CB reduces the degree of density in the original attention maps and increases both the capacity and generalizability of the ViT models. CB incurs negligible costs: 1 line in your model code, no additional parameters, and minimal extra operations.

==> figs/04_arch/architecture.tex <==

\begin{figure*}
  \small
  \centering
  \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figs/04_arch/module.pdf}
    \caption{$\gs$ module}
    \label{fig:our_module}
 \end{subfigure}
  \begin{subfigure}[b]{0.64\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/04_arch/ours_main.pdf}
    \caption{Our vision transformer}
    \label{fig:our_arch}
 \end{subfigure}

  \caption{\small \textbf{Context Broadcasting ($\gs$) module.}
  (a) Our $\gs$ module broadcasts the context to each token.
  (b) The $\gs$ module is inserted at the end of the $\mlp$ block of the Vision Transformer (ViT) architectures. ViTs have other possible positions for our module, but we analyze that inserting at the end of $\mlp$ outperforms others.
  }
  \label{fig:ours}
\end{figure*}


==> figs/05_ablation/ablation.tex <==
\begin{figure}
        \centering
        \includegraphics[width=0.5\linewidth]{figs/05_ablation/entropy_vs_depth_vit-s_ours_legend.pdf}
        
        \begin{subfigure}[b]{0.49\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth]{figs/05_ablation/entropy_vs_depth_cls_vit-s_ours.pdf}
            \vspace{-2em}
            \caption{Layer-wise entropy}
            \label{fig:entropya}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.49\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth]{figs/05_ablation/relative_distance.pdf}
            \vspace{-2em}
            \caption{Relative distance of attention}
            \label{fig:spa_dist}
        \end{subfigure} 
        \vspace{-.75em}
        \caption{\textbf{Attention entropy and relative distance.} We visualize the averaged entropies of the class token and the relative distance of spatial interactions across the layers. 
        % The red dot line is the maximum value of entropy.
        $\gs$ changes the spatial interactions of attention and reserves the long-range dependency.
        }
        \label{fig:entropy}
        \vspace{-1em}
\end{figure}



==> figs/07_heads/heads.tex <==
\begin{table}
    \centering
    % \resizebox{0.6\linewidth}{!}{
    \tabcolsep=0.3cm    
    \small
    \begin{tabular}{c c c c}\\
        \toprule  
        Model & No module & $\gs^\dagger$  & $\gs$ \\
        \midrule
        ViT-Ti & 72.2 & 73.2 & \textbf{73.4}\\
        ViT-S & 79.9 & 80.5 & \textbf{80.8} \\
        ViT-B & 81.8 & 82.0 & \textbf{82.1} \\
        \bottomrule
    \end{tabular}
    % }
    \vspace{-2mm}
    \caption{\textbf{ImageNet-1K performance of $\gs$.} 
    We denote $\gs^\dagger$ as $\gs$ applied to all layers.}
    \label{tab:upper}
    \vspace{-2mm}
\end{table}



==> tabs/10_context.tex <==
% \vspace{ 2mm}
\begin{table}
    \centering
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{c c c c c}
         \toprule
          Architecture & Original & $\gs$ (Average) & Max-pooling & Class token\\
         \midrule
         ViT-S & 79.9 & 80.5 \pos{(+0.6)} & 80.2 \pos{(+0.3)} & 79.3 \nega{($-$0.6)}\\
         \bottomrule
    \end{tabular}}
    \vspace{-2mm}
    \caption{\textbf{ImageNet-1K performance of other context aggregation.} 
    $\gs$, originated from the need for self-attention, is more effective than others.
    % We replace $\gs$ with either max-pooling or the class token. 
    % We show ImageNet-1K top-1 accuracy on the validation set.
    }
    \label{table:gp} 
    % \vspace{-2mm}
\end{table}
